The Training of Neuromodels for Machine Comprehension of Text. Brain2Text Algorithm

Nowadays, the Internet represents a vast informational space, growing exponentially and the problem of search for relevant data becomes essential as never before. The algorithm proposed in the article allows to perform natural language queries on content of the document and get comprehensive meaningful answers. The problem is partially solved for English as SQuAD contains enough data to learn on, but there is no such dataset in Russian, so the methods used by scientists now are not applicable to Russian. Brain2 framework allows to cope with the problem - it stands out for its ability to be applied on small datasets and does not require impressive computing power. The algorithm is illustrated on Sberbank of Russia Strategy's text and assumes the use of a neuromodel consisting of 65 mln synapses. The trained model is able to construct word-by-word answers to questions based on a given text. The existing limitations are its current inability to identify synonyms, pronoun relations and allegories. Nevertheless, the results of conducted experiments showed high capacity and generalisation ability of the suggested approach.

==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%



\begin{thebibliography}
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%

% Online Document
 \begin{enumerate}
\bibitem{latexcompanion} Pranav Rajpurkar, Jian Zhang, Konstantin Lopyrev, Percy Liang.: SQuAD: 100,000+ Questions for Machine Comprehension of Text.(2016) Available via Arxiv. \url{https://arxiv.org/abs/1606.05250. Cited 3 Aug 2017}
\bibitem{latex} Shuohang Wang, Jing Jiang.: Machine Comprehension Using Match-LSTM and Answer Pointer.(2016) Available via Arxiv \url{https://arxiv.org/abs/1608.07905. Cited 3 Aug 2017}
\bibitem{luc} Lutsenko E.V. Conceptual principles of the system (emergent) information theory and its application for the cognitive modelling of the active objects (entities) //2002 IEEE International Conference on Artificial Intelligence System (ICAIS 2002).  
\bibitem{art} A.Artemov, E.Lutsenko, E.Ayunts and I.Bolokhov. Informational Neurobayesian Approach to Neural Networks Training. Opportunities and Prospects.(2017) Available via Arxiv. \url{https://arxiv.org/abs/1710.07264. Cited 3 Nov 2017}

 \end{enumerate}

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
\end{thebibliography}
